Compatible Recurrent Identities of the Sandpile Group and Maximal Stable Configurations

In the abelian sandpile model, recurrent chip configurations are of interest as they are a natural choice of coset representatives under the quotient of the reduced Laplacian. We investigate graphs whose recurrent identities with respect to different sinks are compatible with each other. The maximal stable configuration is the simplest recurrent chip configuration, and graphs whose recurrent identities equal the maximal stable configuration are of particular interest, and are said to have the complete maximal identity property. We prove that given any graph $G$ one can attach trees to the vertices of $G$ to yield a graph with the complete maximal identity property. We conclude with several intriguing conjectures about the complete maximal identity property of various graph products.

==> Paper/Flow-firing.tex <==
\section{Flow-firing}\label{section:flow-firing}
Chip-firing can be thought of as acting on a simplicial complex, where chips are on 0-dimensional cells (vertices) and fired through 1-dimensional cells (edges).
This naturally leads to the generalization of chip-firing into higher dimensions, as done in \cite{duval2013critical}.
\textbf{Ridge-firing}, as explained in \cite{felzenszwalb2019flow}, works over a polytopal decomposition of $n$-dimensional space, where values are assigned to $(n-1)$-dimensional cells (\textbf{ridges}) and rerouted through $n$-dimensional cells (\textbf{facets}).
The first generalization of chip-firing into ridge-firing is the two-dimensional form of ridge-firing, or \textbf{flow-firing}, which works on a planar graph with \textbf{flow} on 1-dimensional cells (edges), which are rerouted through 2-dimensional cells (faces).
We refer readers to \cite{felzenszwalb2019flow} for detailed background on flow-firing.

Flow-firing does not universally display \textbf{global confluence}, meaning each initial configuration can terminate and must terminate at only one stable configuration, or even terminating behavior, but as demonstrated in \cite{felzenszwalb2019flow}, for a \textbf{conservative} configuration, where the inflow equals the outflow at all vertices, the flow-firing process will terminate; moreover, all conservative configurations yield a face representation, or a representation of the flow via values assigned to each face corresponding to the local clockwise flow around the face.
Furthermore, as illustrated in \cite{felzenszwalb2019flow}, a \textbf{pulse}, or an initial configuration where the initial flow in face representation is confined to a single face, is over a topological hole on a planar graph, the configuration will display global confluence.
We extend the idea of conservative initial configurations around a topological hole on planar graphs to allow for multiple topological holes. The flow at a face $F$ is denoted $\operatorname{flow}(F)$.

We define a \textbf{pulse} of \textbf{force} $n\in\mathbb{Z}$ to be the conservative initial configuration that has a flow of $n$ on the removed (also referred to as the distinguished) face whose absence forms a topological hole in the planar graph.  

\begin{definition}\label{definition: confluence}
    A (conservative) initial configuration displays \textbf{local confluence} if it satisfies the \textbf{diamond lemma}: that is, if for all successors of the initial configuration, a configuration $c$ after one step may be either $c_1$ or $c_2$, then there exists a $c_3$ that can be reached from one step from both $c_1$ and $c_2$.
    
    A planar graph displays local confluence if every conservative initial configuration on the planar graph displays local confluence.
    
    A planar graph displays global confluence if every conservative initial configuration on the planar graph displays global confluence.
\end{definition}

It is known that an initial configuration that terminates and displays local confluence must display global confluence, and thus a planar graph that displays local confluence must display global confluence as well.

We assume that in any conservative initial configuration there are always finitely many faces with nonzero flow.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Unidirectional Flow-firing}\label{subsection: unidirectional flow-firing}
\begin{definition}\label{definition:unidirectional flow-firing}
    A \textbf{unidirectional flow-firing configuration} is an initial conservative configuration on a planar graph isomorphic to the $\mathbb{N}$ lattice (a 1-dimensional lattice of square faces enumerated uniquely with the nonnegative integers such that two faces share an edge if their corresponding numbers are consecutive).
    
    The \textbf{sequence of flow} of a unidirectional flow-firing configuration is the sequence formed by taking the flows of the faces with the $i$th term (0 indexed) corresponding to the flow of face $i\in \mathbb{N}$.
\end{definition}

\begin{lemma}\label{lemma: unidirectional flow-firing diamond lemma}
    A unidirectional flow-firing configuration with nonnegative flow at all faces and with a weakly decreasing sequence of flow satisfies the diamond lemma.
\end{lemma}
\begin{proof}
    First we notice that if the sequence of flow is weakly decreasing, no face $k$ can fire towards the face $k-1$, so if it can fire it can only fire to $k+1$.
    Furthermore, if a face $k$ fires towards face $k+1$, the sequence of flow remains weakly decreasing as the flow at face $k$ decreases and the flow at face $k+1$ increases, while the flow at face $k$ was initially at least 2 greater than the flow at face $k+1$ so that boundary remains weakly decreasing.
    Hence, the faces can only fire in the positive direction.
    
    Say we have a configuration $c$ that has (at least) two successors $c_1$ and $c_2$ after one step, meaning that $c$ has at least 2 options to fire. That means for two distinct values of $k$, $\operatorname{flow}(k+1)-\operatorname{flow}(k)\geq 2$. If these two values of $k$, $k_1$ and $k_2$, are at least 2 apart, then their firings do not affect each other, so if $k_1$ fires, then $k_2$ can fire afterwards, satisfying the diamond lemma. If $k_1$ and $k_2$ are consecutive, then firing one will increase the difference of the other, meaning that it still can fire, hence satisfying the diamond lemma. Thus a unidirectional flow-firing configuration with nonnegative flow at all faces and with a weakly decreasing sequence of flow satisfies the diamond lemma.
\end{proof}

\begin{proposition}\label{prop: unidirectional flow-firing constant to pyramid}
    A unidirectional flow-firing configuration with constant nonnegative flow $f\in \mathbb{N}$ for the first $n\in \mathbb{N}$ faces followed by 0 flow on all faces onward will stabilize in a weakly decreasing sequence of flow where the at most one pair of consecutive faces have the same flow, except faces that still have flow $f$, and all other pairs have a difference of 1 flow.
\end{proposition}
For example, a unidirectional flow-firing configuration with sequence of flow 6, 6, 6, 6, 6, 0, \dots~will stabilize to 6, 6, 5, 4, 3, 3, 2, 1, 0, \dots.
\begin{proof}
    We merely need to show such a configuration is reachable, as the unidirectional flow-firing configuration has local confluence and thus global confluence by \ref{lemma: unidirectional flow-firing diamond lemma}, meaning this stable configuration is the unique stabilization.
    The configuration is stable, and by incrementally building a pyramid by firing the outermost face of flow $f$, the ending shape is any unused $f$'s, followed by the pyramid with additional flow starting from the bottom of the pyramid, forming the one pair of consecutive faces with the same flow.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiple Pulses}\label{subsection: multiple pulses}

For a planar graph with $n$ holes $h_1, \dots, h_n$ each with a pulse of force $p_1, \dots, p_n$, respectively, the flow-firing process proceeds as if each hole was the only hole in the planar graph, with specific interactions at overlaps of the supports of each pulse.

If the holes of two pulses share an edge and are of differing force, then there is a flow through the edge between them, but the edge has no way to fire.
This edge thus will not fire, and it need not be taken into consideration for the stability of a flow-fire configuration, but is critical to maintain the conservativity of a configuration.

\begin{definition}\label{definition: support}
The \textbf{support} of a pulse of nonzero force is the union of the faces that, if the location of the pulse was the only hole in the planar graph, would have a nonzero flow through it in the final configuration.
The support of a pulse of zero force is the union of the faces that share an edge with the hole of the pulse.
\end{definition}
The support of any configuration is the set of faces that have nonzero flow through them.
There are three \textbf{signs} of pulses: positive, negative, and zero, which directly corresponds to the sign of the force of the pulse.
We use the convention that a positive sign is opposite to a negative sign, but a sign of 0 is not opposite to any sign.
Note that if exactly one of two signs is zero, then the signs are differing but not opposite.
\begin{definition}\label{def:Aztec pyramid}
The \textbf{Aztec pyramid} of a nonnegative pulse of force $p$ is the configuration where each undistinguished face $F$ has $\max{p-d+1,0}$ flow, where $d$ is the distance of $F$ from the pulse, or the minimal number of edges that must be crossed (one may not cross through vertices) to reach $F$ from the distinguished face.
The hole still has $p$ flow.
The flow through a face $F$ in the Aztec pyramid configuration of pulse $p$ is denoted by $\operatorname{Aztec}_p(F)$ or simply $\operatorname{Aztec}(F)$ if which pulse is being referred to is obvious.
The Aztec pyramid of a negative pulse of force $-p$ is the configuration where each face $F$ has flow $-\operatorname{Aztec}_p(F)$.
\end{definition}

It has been demonstrated in \cite{felzenszwalb2019flow} that the terminating configuration of a pulse with force $p$ is its Aztec pyramid.

If none of the supports overlap or share an edge, the flow-firing process will terminate, with the final configuration in each support being the final configuration if the location of the pulse was the only hole in the planar graph, and 0 flow on all the other faces.

If any supports share an edge or overlap, the interactions of the flow-firing process are as follows:
\begin{itemize}
    \item The supports of multiple pulses overlap (share a face)
    \begin{itemize}
        \item If the supports of any two pulses of differing signs overlap, the flow-firing process will not terminate as the final configurations of the two individual pulses do not agree at at least one face, and each pulse will continue the flow-firing process towards its final configuration.
        \item If the overlapping supports' pulses are of the same sign, then the flow-firing process will terminate unless other supports' interactions cause it to fail to terminate. If it terminates, the final flow for any face that is part of multiple supports, say of pulses $p_1$, $p_2$, \dots, $p_n$, is the $\operatorname{Aztec}_{p_i}(F)$ for which $\left|\operatorname{Aztec}_{p_i}(F)\right|$ is maximized among all $1 \leq i \leq n$.
    \end{itemize}
    \item The supports of multiple pulses share an edge
    \begin{itemize}
        \item If the supports of any two pulses of opposite signs share an edge, the flow-firing process will not terminate as one face containing that edge will have a positive flow and the other a negative flow, meaning that the flow-firing would not be able to terminate, as it would attempt to balance the two faces, but then the pulses would return the face to its previous value.
        \item If the supports of any two pulses of non-opposite signs share an edge, the flow-firing process will terminate unless other supports' interactions cause it to fail to terminate. The two pulses do not impact each other's supports in any way.
    \end{itemize}
\end{itemize}

This should be able to generalize to higher dimensional complexes, using the ridge-firing process as defined in \cite{felzenszwalb2019flow}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Conservative Flows and Multiple Holes}\label{subsection: conservative flows}

If a conservative flow may encompass holes but also faces, then there is no guarantee that the process will have global confluence (for example, take the infinite planar graph of the 2-dimensional lattice of $\mathbb{Z}^2$ with three consecutive face flows of 2 in a line, with a hole at one of the end 2s; the other end 2 will cause a 1 to be outside of the support of the pulse, but it can be in 3 different locations, thus creating at least 3 different final configurations). Essentially, if the starting configuration has flow that enables it to put flow outside of all of the pulses' supports, then the process will not have global confluence as the choices made outside of the supports create different final configurations. The flowfire process may or may not terminate depending on the pulses.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Conservative Flows and a Single Hole}\label{subsection: conservative flows and a single hole}
\begin{lemma}\label{lemma: < aztec = global confluence}
    If the initial configuration has the flow of each face $F$ bounded between 0 and $\operatorname{Aztec}(F)$, then the initial configuration exhibits global confluence.
\end{lemma}
\begin{proof}
    At no face can the configuration ever exceed the Aztec pyramid configuration. Because of this, as the pulse must terminate at a configuration no less than the Aztec pyramid at any face, regardless of the order of firing the configuration will terminate at the Aztec pyramid.
\end{proof}

\begin{proposition}\label{proposition: single > aztec}
    If the initial conservative flow configuration has nonnegative flow through all faces and either contains exactly one face $F$ in the support of the pulse with flow equal to $\operatorname{Aztec}(F)+1$, or a flow outside the support of magnitude at least 2, with all other faces $F$ with flow no more than $\operatorname{Aztec}(F)$, then the initial conservative flow does not exhibit global confluence.
\end{proposition}
\begin{proof}
    In the case that flow is outside the support, it has at least 2 places that it can flow to, thus able to violate global confluence.
    
    In the case that the flow is inside the support, either the face is in the same row or column of the hole, or it is not.
    If it is not, create the Aztec pyramid at all faces except that face by using the hole, and then let that face's flow run down the Aztec pyramid, where it has at least 2 places that it can flow to, thus able to violate global confluence.
    
    If the flow is inside the support and in the same row or column of the hole, then without loss of generality it is to the right of the hole (so in the same row).
    Then, the Aztec pyramid in that row, to the right of the face that is greater than the Aztec pyramid configuration, cannot be formed without firing that face.
    However, this configuration still violates global confluence, as everywhere else the Aztec pyramid can be made, and thus the flow in that face can travel up or down, at which point it may continue down the Aztec pyramid, where it has at least 2 places that it can flow to, thus able to violate global confluence.
\end{proof}

Notice that the first condition in \cref{proposition: single > aztec} cannot be generalized to if there exists a face $F$ in the support of the Aztec pyramid such that $\operatorname{flow}(F)>\operatorname{Aztec}(F)$, as the initial configuration
\begin{center}
    \begin{tabular}{*7{c}}
         0&0&0&1&0&0&0\\
         0&0&\textbf{3}&2&1&0&0\\
         0&1&2&3&2&1&0 \\
         \cline{4-4}
         1&2&3&\multicolumn{1}{|c|}{3}&3&2&1\\
         \cline{4-4}
         0&1&2&3&2&1&0\\
         0&0&1&2&1&0&0\\
         0&0&0&1&0&0&0\\
    \end{tabular}
\end{center}
where the hole is the boxed 3, has one face with flow greater than it would in the Aztec pyramid configuration.
This face can only fire to the left or up, and once it does one of these the only remaining option is to fire in the other of the two options, resulting in the terminating configuration
\begin{center}
    \begin{tabular}{*7{c}}
         0&0&1&1&0&0&0\\
         0&1&1&2&1&0&0\\
         0&1&2&3&2&1&0 \\
         \cline{4-4}
         1&2&3&\multicolumn{1}{|c|}{3}&3&2&1\\
         \cline{4-4}
         0&1&2&3&2&1&0\\
         0&0&1&2&1&0&0\\
         0&0&0&1&0&0&0\\
    \end{tabular}
\end{center}
and hence demonstrating that this initial configuration displays global confluence.

%Not including Uniform Conservative Flows and a Single Hole subsection

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Single Pulse of Nontrivial Radius}\label{subsection: single pulse of nontrivial radius}
Define a pulse of \textbf{radius} $r\in\mathbb{Z}_{>0}$ and force $f$ to be the initial configuration with flow $f$ through all faces that are a distance at most $r$ away from the hole.

\begin{proposition}\label{proposition:Z2 grid pulse radius global confluence}
    On the $\mathbb{Z}^2$ lattice, a pulse of radius $r$ and force $f$ exhibits global confluence iff $|f|\leq 1$ or $r\leq 1$.
\end{proposition}
\begin{proof}
    If $|f|\leq 1$, then the pulse is already stable, and thus exhibits global confluence.
    
    If $r \leq 1$, then the initial configuration is less than or equal to the Aztec pyramid of the pulse, and thus by \cref{lemma: < aztec = global confluence}, the final configuration must be the Aztec pyramid, implying global confluence.
    
    If $|f| \geq 2, r \geq 2$, without loss of generality let $f \geq 2$.
    If $f=2$, we see the result as the $4r$ outermost faces ($r$ away from the hole) have multiple options for firing, and once all of them have stabilized (which they will as there can be at most $4r$ firings), the configuration is stable.
    Hence as there were multiple options for the ending stable configuration, it does not display global confluence.
    We now assume $f \geq 3$.
    
    We will show that for $r \leq \frac{f+1}{2}$, the pulse does not display global confluence.
    We will first show that there exists a firing sequence that turns the pulse of radius $r$ into a configuration less than or equal to the Aztec pyramid, and thus the Aztec pyramid is a possible terminating configuration.
    We will first prove that there exists a way to have the squares directly to the right of the hole be less than the Aztec pyramid without changing the flow through any other of the faces. We note that starting from the square immediately to the right of the hole and continuing right, in order for the final configuration to be stable, the flows through those faces must form a weakly decreasing sequence starting at $f$ and ending at 0, where each decreasing step can only go down by 1.
    Hence, any stable configuration on those faces must have at least $f+(f-1)+\cdots+2+1+0=\frac{f(f+1)}{2}$ total flow. We fire the faces directly to the right of the hole towards the right until they, by themselves, are stable relative to each other. As the flow is conserved, there is a total of $rf$ flow.
    But if $rf\leq \frac{f(f+1)}{2}$, or equivalently $r \leq \frac{f+1}{2}$, then once it stabilizes it must be less than or equal to the Aztec pyramid. We apply this firing sequence similarly to the faces directly above, below, and to the left of the hole as well.
    Furthermore, using the same logic for the faces with flow off the axis, for example quadrant I could all fire to the right, the entire pulse of radius $r$ can be stabilized.
    In that case, at a y-coordinate of $n$, the total flow would be $rf-nf$, where the total flow in the Aztec pyramid would be $\frac{f(f+1)}{2}-f-(f-1)-\cdots-(f-n+1) \geq \frac{f(f+1)}{2}-nf$, so for those cases it results in a configuration less than or equal to the Aztec pyramid once stabilized (this is because such a weakly decreasing line of faces exhibits local confluence, and one can make the faces build the Aztec pyramid and stop when it runs out of flow).
    Hence, there exists a firing sequence that takes the pulse of radius $r$ into a configuration less than or equal to the Aztec pyramid, and thus the Aztec pyramid is a possible terminating configuration.
    Now we will show that there exists a successor of the pulse of radius $r$ that has flow outside of the support of the Aztec pyramid. Stabilize the pulse of radius $r$, except do not fire $(1,1)$.
    The resulting configuration for all of the faces except $(1,1)$ must be greater than or equal to the Aztec pyramid. If it is greater than the Aztec pyramid, then there must be flow outside of the support of the Aztec pyramid.
    If it is equal to the Aztec pyramid, then by Proposition \ref{proposition: single > aztec}, there exist terminating configurations that have a support that is a strict superset of the support of the Aztec pyramid.
    
    \begin{figure}
        \centering
        \includegraphics{Pictures/Prop8-8Ex.JPG}
        \caption{Example diagram for $\protect{f=7,r=6}$ (the hole is the bolded 7). From left to right: (1) firing $\protect{x=\pm1}$ upwards ; (2) final configuration after firing central column downwards from (1); (3) firing $(0,r)$ to the left and right, with the flow cascading upwards from (1); final configuration after firing central column downwards from (3).}
        \label{fig:Prop8-8Ex}
    \end{figure}
    
    We will now prove the $r > \frac{f+1}{2}$ cases by considering the parity of $f$.
    
    For odd flow $f$, fire the faces with $x=\pm 1$ in the positive $y$ half of the lattice upwards. By Proposition \ref{prop: unidirectional flow-firing constant to pyramid}, this will use the uppermost $\frac{f-1}{2}$ squares of flow $f$ and create a pyramid going from $f-1$ at $(\pm 1, r - \frac{f-1}{2})$ to 1 at $(\pm 1, r + \frac{f-1}{2}-1)$.
    The two squares $(\pm 1,r)$ have flow $\frac{f-1}{2}$. If $f\geq 5$, then the square $(0,r)$ with $f$ flow may fire to the left and right once, allowing those flows to cascade upwards and reach squares $(\pm 1, r + \frac{f-1}{2})$.
    The squares from $(0,r - \frac{f-1}{2})$ to $(0,r-1)$, still with flow $f$, along with the square $(0,r)$ with flow $f-2$ by Proposition \ref{prop: unidirectional flow-firing constant to pyramid} will form a pyramid from $(0,r - \frac{f-1}{2})$ to $(0, r + \frac{f-1}{2})$ starting with $f-1$ flow and going down to 1 flow, with the double flow at flow $f-2$.
    Hence, this configuration will have positive flow at the three squares from $(-1,r + \frac{f-1}{2})$ to $(1,r + \frac{f-1}{2})$.
    However, if we merely fire those three columns purely upwards and then outwards to the left and right as necessary, the squares $(\pm 1, r + \frac{f-1}{2})$ will have 0 flow through them as the vertical firing by Proposition \ref{prop: unidirectional flow-firing constant to pyramid} will only yield a pyramidal flow from flow $f-1$ at $(\pm 1, r - \frac{f-1}{2}$ to flow 1 at $(\pm 1, r + \frac{f-1}{2} - 1)$.
    From this configuration it is possible for flow to never reach those squares; if the other columns are fired upwards initially, then each column at $x=\pm a$ for $a\leq r - \frac{f-3}{4}$ will be able to reach $(\pm a, r + \frac{f-1}{2} - a)$, but no further, as afterwards any firing is only to the left or right, meaning it is not possible to have flow go through $(\pm 2, r + \frac{f-1}{2})$ and then inwards to $(\pm 1, r \frac{f-1}{2})$ (alternatively, another way to look at this is that the flow configuration now is less than or equal to the Aztec pyramid with $r + \frac{f-1}{2}$ flow at the hole at the origin if the same firing process is done on the lower half of the lattice firing downwards, meaning that by the proof of Lemma \ref{lemma: < aztec = global confluence}, flow cannot reach the squares $(\pm 1, r + \frac{f-1}{2})$, which are outside of the Aztec pyramid's support.)
    Hence for odd flow $f \geq 5$ with $r \geq \frac{f+1}{2}$, the pulse of flow $f$ and radius $r$ does not have global confluence. For flow $f=3$, there is not sufficient flow for the square $(0,r)$ to fire both to the left and right, but there is sufficient to fire to one of the two, without loss of generality to the right, and the proof still holds as that one flow will reach $(1,r)$, which is not possible when all three columns fired upwards first.
    This proof works as long as the hole does not interfere with the aforementioned process, or when $r \geq \frac{f+1}{2}$. Combined with the proof for $r \leq \frac{f+1}{2}$, this completes the proof for odd $f$.
    
    For even flow $f\geq 4$, fire the faces with $x=\pm 1$ in the positive $y$ half of the lattice upwards. By Proposition \ref{prop: unidirectional flow-firing constant to pyramid}, this will use the uppermost $\frac{f}{2}$ squares of flow $f$ and create a pyramid going from $f-1$ at $(\pm 1, r - \frac{f}{2})$ to 1 at $(\pm 1, r + \frac{f}{2}-1)$, with the double flow at flow $\frac{f}{2}$ at $(\pm 1, r-1)$ and $(\pm 1, r)$.
    The two squares $(\pm 1, r)$ have flow $\frac{f}{2}$, with the pyramid without any double flows onward from that point. If $f\geq 6$, the square $(0,r)$ can fire to the left and then the right, and the proof follows similar to the odd flow $f \geq 5$ case aforementioned.
    If $f=4$, there is only sufficient flow at $(0,r)$ to fire either to the left or right but not both, and the proof follows similar to the odd flow $f=3$ case.
    The proof works as long as the hole does not interfere with the aforementioned process, or when $r > \frac{f}{2}$. Combined with the proof for $r \leq \frac{f+1}{2}$, this completes the proof for even $f$.
    
    This completes the proof.
    %We will prove the result by induction on $r$. First, we prove the base case of $r=2$. Of the 8 outer faces, fire 7 of them in a way that no two faces fire to the same location (a simple method would be to fire north if possible, otherwise east if possible, and otherwise south if possible. Now we only have 1 face $F$ that is greater than $\operatorname{Aztec}(F)$, and by Proposition \ref{prop: single > aztec}, the configuration does not have global confluence, as we make the Aztec pyramid and let the face flow down. For simplicity, let the eighth outer face not be in the same row or column as the hole. For the inductive step, assume the result holds for $r=k$. We will show the result holds for $r=k+1$.
\end{proof}
